Build Code Needs Maintenance Too: A Study on Refactoring and Technical Debt in Build Systems

In modern software engineering, build systems play the crucial role of facilitating the conversion of source code into software artifacts. Recent research has explored high-level causes of build failures, but has largely overlooked the structural properties of build files. Akin to source code, build systems face technical debt challenges that hinder maintenance and optimization. While refactoring is often seen as a key tool for addressing technical debt in source code, there is a significant research gap regarding the specific refactoring changes developers apply to build code and whether these refactorings effectively address technical debt. In this paper, we address this gap by examining refactorings applied to build scripts in open-source projects, covering the widely used build systems of Gradle, Ant, and Maven. Additionally, we investigate whether these refactorings are used to tackle technical debts in build systems. Our analysis was conducted on \totalCommits examined build-file-related commits. We identified \totalRefactoringCategories build-related refactorings, which we divided into \totalCategories main categories. These refactorings are organized into the first empirically derived taxonomy of build system refactorings. Furthermore, we investigate how developers employ these refactoring types to address technical debts via a manual commit-analysis and a developer survey. In this context, we identified \totalTechnicalDebts technical debts addressed by these refactorings and discussed their correlation with the different refactorings. Finally, we introduce BuildRefMiner, an LLM-powered tool leveraging GPT-4o to automate the detection of refactorings within build systems. We evaluated its performance and found that it achieves an F1 score of \toolFoneScore across all build systems.

==> Images/Refactored_Code.tex <==
\begin{figure}[ht!]
\centering
\vspace{-0.4cm}
\caption*{Number of Interviewees Mentioning Each Criterion}

\begin{bchart}[step=1,max=10,width=2.8cm]
%\bcxlabel{number of employees}
\bcbar[label=Dependencies]{5}
\bcbar[label=Readability]{4}
\bcbar[label=Well-defined APIs]{4}
\bcbar[label=Extensibility]{4}
\bcbar[label=Performance]{3}
\bcbar[label=Code Size]{3}
\bcbar[label=Design Principles]{3}
\bcbar[label=Ease of Testing]{3}
\bcbar[label=Code Complexity]{2}





\end{bchart}
    \vspace{-0.4cm}
\caption{Criteria mentioned by interviewees that address the state of refactored code (10 interviewees). \wajdi{I created this maybe you find it better in presentation.}}
    \vspace{-0.4cm}
    \label{fig:interview_code_criteria}
\end{figure}

==> Listings/RefactoringExamples/name.tex <==
\begin{lstlisting}[language=diff,caption={A},label={lst:a},numbers=left,frame=lines, escapechar=\!]

	!\RedL! <target name="init">
	!\RedL!	<mkdir dir="${bin}"/>
	!\RedL!	<mkdir dir="${dist}"/>
	!\RedL!	<mkdir dir="${doc}"/>
        !\RedL!	</target>

	<target name="clean">
        <delete dir="${bin}"/>
	<delete dir="${dist}"/>
	<delete dir="${doc}"/>
	</target>

	!\GreenL!<target name="init" depends="clean">
	!\GreenL!	<mkdir dir="${bin}"/>
	!\GreenL!	<mkdir dir="${dist}"/>
	!\GreenL!	<mkdir dir="${doc}"/>
	!\GreenL!</target>

\end{lstlisting}

==> Tables/Tools_Examples.tex <==
\begin{table*}
\begin{tabularx}{\textwidth}{lX}
\toprule
\textbf{Criteria} & \textbf{Examples} \\
\midrule
Change size & (1) Tool [12] minimizes code changes required to fix design defects.\\
            & (2) Tool [22] suggests refactoring solutions that represent a good trade-off between minimizing code smells and improving QMOOD while minimizing the number of refactorings.\\ \hline
%%%%%%%%%%%%%%%%%%%%%
Cost/time & (1) Tool[7] generates recommendations that reduce problematic dependencies while reducing the effort required for this kind of architecture improvement by two-thirds. \\ \hline
%%%%%%%%%%%%%%%%%%%%%
Propagation of changes & (1) Interviewees[1],[4], and [5] suggest minimizing refactoring's knock-on effects on other classes, teams, and architectural elements when refactoring. \\ \hline
%%%%%%%%%%%%%%%%%%%%%
Unchangeable code &  (1) Interviewee[3] suggests avoiding changing safety-critical code when refactoring.  \\ \hline
%%%%%%%%%%%%%%%%%%%%
Code complexity & (1) Tool[1] suggests resolving the \textit{Long Method} code smell in an effort to reduce its complexity. \\
                & (2) Tool[23] recommends several refactoring solutions to remove the \textit{Brain Method} code smell, known as a long and complex method. \\
                & (3) Tool[22] suggests a list of best refactoring solutions to improve QMOOD (Quality Model for Object-Oriented Design) quality metrics such as \textit{Understandability} where The code complexity is encoded in its Computation equation. \\ \hline
%%%%%%%%%%%%%%%%%%%%%
Code size & (1) Tool[5] increase clone maintenance support by unifying clone detection and keeping code size down. \\
          & (2) Tool[19] recommends removing quality defects such as code clones and long methods. \\ \hline
%%%%%%%%%%%%%%%%%%%%%          
Design principles & (1) Tool[27] favor splitting a class with different responsibilities into several classes to find a balance between its cohesion and coupling by considering the Conceptual and semantic Similarity between Methods. \\
                  & (2) Tool[18] detects \textit{Feature Envy} code smell  
instances-defined as occurring when a method calls methods on another class more times than on the source class- and then identifies Move Method refactorings to fix them. \\ 

                  & Tool[16] proposes an architectural repair recommendation system whose main purpose is to provide refactoring guidelines for developers and maintainers when fixing violations in the module architecture view of object-oriented systems.                          \\ \hline
%%%%%%%%%%%%%%%%%%%%%
Dependencies & (1) Tool[28] favors changes that reduce coupling between classes. \\
             & (2) Tool[10] recognize opportunities for extracting cohesive classes from \textit{God Classes}. \\ \hline
%%%%%%%%%%%%%%%%%%%%%
Ease of testing & (1) Tool[2] propose a refactoring process towards a design that minimizes the number of unit test cases for each class in the system.  \\ \hline
%%%%%%%%%%%%%%%%%%%%%
Extensibility & (1) Tool[11] recognize opportunities for extracting cohesive classes from \textit{God Classes} for better extensibility of the code.\\
              & (2) Tool[8] suggests improving different quality attributes (e.g., Extensibility, etc.) from the QMOOD model.\\ \hline
%%%%%%%%%%%%%%%%%%%%%
Performance & (1) Interviewee[8] suggests refactoring to improve performance by using cache and avoiding the cost of re-computing. \\ \hline
%%%%%%%%%%%%%%%%%%%%%
Readability & (1) Tool[29] suggests fixing\textit{ Method Naming Convention} problems by requesting more meaningful names from developers.\\
            & (2) Tool[1] improves the elimination of code smells \textit{Long Method}, \textit{Large Class}, and \textit{Lazy Class} such as a means to improve the readability and comprehensibility of existing software.\\
%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabularx}
\caption{Examples of how tools address criteria that focus on the refactoring activity itself.}
\label{table:process_tools}
\end{table*}



%% Old version

% \begin{table}
% \begin{tabularx}{\columnwidth}{lX}
% \toprule
% \textbf{Criteria} & \textbf{Examples} \\
% \midrule
% Change size & 
% \begin{enumerate}
%     \item Tool [12] minimizes code changes required to fix design defects.
%     \item Tool [22] suggest refactoring solutions that represents a good trade-off between minimizing code-smells and improving QMOOD while minimizing the number of refactorings. \end{enumerate} \\
% Cost/time & \begin{enumerate}
%     \item Tool[7] generates
% recommendations that reduce problematic dependencies while reducing the effort required for this kind of architecture improvement by two-thirds. \end{enumerate}\\
  
% Propagation of changes & \begin{enumerate}
%     \item Interviewees[1],[4] and [5] suggest minimizing refactoring's knock-on effects on other classes, teams, and architectural elements when refactoring. 
%     \end{enumerate} \\

% Unchangeable code &  \begin{enumerate}
%     \item Interviewee[3] suggests avoiding changing safety-critical code when refactoring. \end{enumerate} \\
% \bottomrule
% \end{tabularx}
% \caption{Examples of how tools address criteria that focus on the refactoring activity itself.}
% \label{table:process_tools}
% \end{table}

% \begin{table}
% \begin{tabularx}{\columnwidth}{lX}
% \toprule
% \textbf{Criteria} & \textbf{Examples} \\
% \midrule
% Code complexity & \begin{enumerate}
%     \item Tool[1] suggests resolving the \textit{Long Method} code smell in an effort to reduce its complexity. 
%     \item Tool[23] recommends several refactoring solutions to remove the \textit{Brain Method} code smell, known as a long and complex method. 
% \end{enumerate}
% \\
% Code size & \begin{enumerate}
% \item Tool[5] increase clone maintenance support by unifying clone detection and keeping code size down. 
% \item Tool[19] recommends removing quality defects such as code clones and long methods.

% \end{enumerate} \\
% Design principles & \begin{enumerate} 
% \item Tool[27] favor splitting a class with different responsibilities into several classes to find a balance between its cohesion and coupling by considering the Conceptual and semantic Similarity between Methods. 
% \item Tool[18] detects \textit{Feature Envy} code smell
% instances and then identify Move Method refactorings to fix them.
% \end{enumerate}
% \\
% Dependencies & \begin{enumerate}
% \item Tool[28] favors changes that reduce coupling between classes  
% \item Tool[10] recognize opportunities for extracting cohesive classes from \textit{God Classes} 
% \end{enumerate}
% \\
% Ease of testing & \begin{enumerate}
%     \item Tool[2] propose a refactoring process towards a design that minimizes the number of unit test cases for each class in the system.  \end{enumerate}\\
% Extensibility & \begin{enumerate} 
%     \item Tool[11] recognize opportunities for extracting cohesive classes from \textit{God Classes} for a better extensibility of the code
%     \item Tool[8] suggests improving different quality attributes (e.g., Extensibility, etc.), from the QMOOD model
%     \end{enumerate}
%     \\
% Performance & \begin{enumerate}
%     \item Interviewee[8] suggests refactoring to improve performance by using cache and avoiding the cost of re-computing \end{enumerate}\\
% Readability & \begin{enumerate}
%     \item Tool[29] suggests fixing\textit{ Method Naming Convention} problems by requesting  more meaningful names from developers
%     \item Tool[1] improves the elimination of code smells \textit{Long Method}, \textit{Large Class}, and \textit{Lazy Class} such as a means to improve the readability and comprehensibility of existing software
%     \end{enumerate} \\
% Well-defined APIs & \begin{enumerate}
%     \item Tool[8] suggests improving the classes' functionality that is accessible via their public interfaces. \end{enumerate} \\
% \bottomrule
% \end{tabularx}
% \caption{Examples of how tools address criteria that focus on the qualities of refactored code.}
% \label{table:code_tools}
% \end{table}

==> Tables/Tools_Questions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
\centering
\caption{Criteria for evaluating refactoring recommendation tools. }
\vspace{-0.3cm} 
\resizebox{\columnwidth}{!}{%
\label{tab:digital_libraries}
\begin{tabular}{|l|l|}\hline
\rowcolor{gray!60}\multicolumn{1}{|c|}{\textbf{Question}} & \multicolumn{1}{c|}{\textbf{Yes/No}} \\ \hline
Does academic publication/website propose a tool?  &  Yes  \\ \hline
\rowcolor{gray!30} Does the tool solely focus on implementing refactoring?                 &  No     \\ \hline
Does the tool provide clear "how to refactor" recommendations, & Yes \\ 
rather than primarily focusing on where to refactor?   &  \\ \hline

\rowcolor{gray!30} Are the recommendations provided by the tool unambiguous?                      &  Yes    \\  \hline
Are the recommendations generic and applicable to any part of  &  No \\ 
 the code rather than specific to certain instances?    &        \\ \hline

\end{tabular}
}
\label{tab:Tools_Questions}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
